Edge-aware Consistent Stereo Video Depth Estimation

Video depth estimation is crucial in various applications, such as scene reconstruction and augmented reality. In contrast to the naive method of estimating depths from images, a more sophisticated approach uses temporal information, thereby eliminating flickering and geometrical inconsistencies. We propose a consistent method for dense video depth estimation; however, unlike the existing monocular methods, ours relates to stereo videos. This technique overcomes the limitations arising from the monocular input. As a benefit of using stereo inputs, a left-right consistency loss is introduced to improve the performance. Besides, we use SLAM-based camera pose estimation in the process. To address the problem of depth blurriness during test-time training (TTT), we present an edge-preserving loss function that improves the visibility of fine details while preserving geometrical consistency. We show that our edge-aware stereo video model can accurately estimate the dense depth maps.

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/images/blockdiagram.tex <==
\begin{figure}[tbp]
	\centering
	\includegraphics[width=1\linewidth]{images/ECSV/ECSV.png}
	\caption{Overview of our test-time training (TTT) on stereo video. Here, we show the loss computations for frame $i$. Our model enforces geometric consistency between the left and right image pair ($i_l, i_r$) (red data flow) and between the consecutive frames ($i_l, j_l$) (blue data flow). The computed losses optimize the image-based stereo network. For more details, refer to Sec. \ref{sec:main}.}
	\label{fig:blockdiagram}
\end{figure}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/images/edgeLoss.tex <==
\begin{figure*}[tbp]
	\centering
	\begin{minipage}[t]{\linewidth}
		\centering
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/frame_000018.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/frame_000033.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/frame_000043.png}
	\end{minipage}
	\begin{minipage}[t]{\linewidth}
		\centering
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000018_e0000_iter000000.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000033_e0000_iter000000.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000043_e0000_iter000000.png}
	\end{minipage}
	\begin{minipage}[t]{\linewidth}
		\centering
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000018_e0001_iter000418.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000033_e0001_iter000418.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000043_e0001_iter000418.png}
	\end{minipage}
	\begin{minipage}[t]{\linewidth}
		\centering
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000018_e0002_iter000836.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000033_e0002_iter000836.png}
		\includegraphics[width=0.32\linewidth]{images/cvde_eval/depth_000043_e0002_iter000836.png}
	\end{minipage}
	\caption{Problem of depth blurriness in test-time training process. The top row shows input color frames at different instances from KITTI odometry \cite{Geiger2012CVPR} dataset. Each consecutive row represents predicted depth maps after 0, 1 and 2 epochs, respectively.}
	\label{fig:edge_loss}
\end{figure*}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/images/eth3dGradVis.tex <==
\begin{figure*}[htpb]
	\begin{center}
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.242\linewidth]{images/eth/color_000015.png}
            \includegraphics[width=0.242\linewidth]{images/eth/color_000016.png}
            \includegraphics[width=0.242\linewidth]{images/eth/color_000017.png}
            \includegraphics[width=0.242\linewidth]{images/eth/color_000018.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{RGB images}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.242\linewidth]{images/eth/midas_000015.png}
            \includegraphics[width=0.242\linewidth]{images/eth/midas_000016.png}
            \includegraphics[width=0.242\linewidth]{images/eth/midas_000017.png}
            \includegraphics[width=0.242\linewidth]{images/eth/midas_000018.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{MiDaS \cite{ranftl2019towards}}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.242\linewidth]{images/eth/cvd_000015.png}
            \includegraphics[width=0.242\linewidth]{images/eth/cvd_000016.png}
            \includegraphics[width=0.242\linewidth]{images/eth/cvd_000017.png}
            \includegraphics[width=0.242\linewidth]{images/eth/cvd_000018.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{CVDE \cite{CVDE}}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.242\linewidth]{images/eth/msg_000015.png}
            \includegraphics[width=0.242\linewidth]{images/eth/msg_000016.png}
            \includegraphics[width=0.242\linewidth]{images/eth/msg_000017.png}
            \includegraphics[width=0.242\linewidth]{images/eth/msg_000018.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{CVDE + Multi-scale Gradient Loss}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.242\linewidth]{images/eth/cl_000015.png}
            \includegraphics[width=0.242\linewidth]{images/eth/cl_000016.png}
            \includegraphics[width=0.242\linewidth]{images/eth/cl_000017.png}
            \includegraphics[width=0.242\linewidth]{images/eth/cl_000018.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{CVDE + Contrastive Loss}\end{turn}			
		\end{minipage}	
		\\
		\caption{Sample depth maps on ETH3D dataset. Note how our proposed edge enhancement method preserves the details and creates sharper depth maps.}
		\label{fig:eth3d_grad_vis}
	\end{center}
\end{figure*}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/images/eth3dVclVis.tex <==
\begin{figure*}[h]
	\centering
	\begin{minipage}[c]{1\linewidth}
		\centering
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/color_000025.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/color_000026.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/color_000029.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/color_000030.png}
	\end{minipage}
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\begin{turn}{0}\footnotesize{RGB images}\end{turn}			
	\end{minipage}	
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/midas_000025.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/midas_000026.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/midas_000029.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/midas_000030.png}
	\end{minipage}
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\begin{turn}{0}\footnotesize{MiDaS \cite{ranftl2019towards}}\end{turn}			
	\end{minipage}	
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvd_000025.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvd_000026.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvd_000029.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvd_000030.png}
	\end{minipage}
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\begin{turn}{0}\footnotesize{CVDE \cite{CVDE}}\end{turn}			
	\end{minipage}	
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvd_000025_final.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvd_000026_final.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvde_000029_final.png}
		\includegraphics[width=0.242\linewidth]{images/vcl_eth3d/cvde_000030_final.png}
	\end{minipage}
	\\
	\begin{minipage}[c]{1\linewidth}
		\centering
		\begin{turn}{0}\footnotesize{Ours, $\mathcal{L}^\textit{LR}$, $\mathcal{L}^\textit{T}$}\end{turn}			
	\end{minipage}	
	\\
	\caption{Sample depth maps on ETH3D dataset predicted in rows respectively by: MiDaS, and MiDaS after test-time training with CVDE, with our left-right consistency loss ($\mathcal{L}^\textit{LR}$), and with both $\mathcal{L}^\textit{LR}$ and $\mathcal{L}^\textit{T}$.}
	\label{fig:eth3d_vcl_vis}
\end{figure*}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/images/stereoVis.tex <==
\begin{figure*}[htpb]
	\begin{center}
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/color_000008.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/color_000011.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/color_000014.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{RGB images}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/lea_000008.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/lea_000011.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/lea_000014.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{LEAStereo \cite{cheng2020hierarchical}}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd_000008_CVDE.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd_000011_CVDE.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd_000014_CVDE.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{CVDE \cite{CVDE}}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/vcl_000008.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/vcl_000011.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/vcl_000014.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{Ours, $\mathcal{L}^\textit{LR}$}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd_000008.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd_000011.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd_000014.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{Ours, $\mathcal{L}^\textit{T}$}\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd+cl_000008.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd+cl_000011.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd+cl_000014.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{Ours, $\mathcal{L}^\textit{T}$, $\mathcal{L}^\textit{C}$ }\end{turn}			
		\end{minipage}	
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd+cl_000008_C.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd+cl_000011_C.png}
			\includegraphics[width=0.32\linewidth]{images/stereo/cvd+cl_000014_C.png}
		\end{minipage}
		\\
		\begin{minipage}[c]{1\linewidth}
			\centering
			\begin{turn}{0}\footnotesize{\textbf{ECSV}: Ours, $\mathcal{L}^\textit{T}$, $\mathcal{L}^\textit{C}$, $\mathcal{L}^\textit{LR}$}\end{turn}			
		\end{minipage}	
		\\
		\caption{Visualization of depth maps on the KITTI odometry dataset for sample consecutive frames. The last row show our the estimated depth maps by our \textbf{E}dge-aware \textbf{C}onsistent \textbf{S}tereo \textbf{V}ideo (\textbf{ECSV}) model.}
		\label{fig:stereo_vis}
		\vspace{-0.5 cm}
	\end{center}
\end{figure*}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/images/trajectory.tex <==
\begin{figure*}[h]
	\centering
	\includegraphics[width=0.495\linewidth]{images/traj/colmap_orb_comaprison_trajectories.png}
	\includegraphics[width=0.495\linewidth]{images/traj/colmap_orb_comaprison_xyz_view.png}
	\caption{Trajectories of COLMAP vs. ORB-SLAM2 for a sequence of KITTI dataset. The projections of trajectories on $xz$-plane (\emph{Left}) and on $x$-, $y$- and $z$-axis (\emph{Right}).}
	\label{fig:traj_comparison}
\end{figure*}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/tables/colmapOrb.tex <==
\begin{table}[h]
	\centering
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{lcccc}
			\toprule
			& Time ($s$) & Mean error ($m$) & Median error ($m$) & RMSE ($m$)  \\
			\midrule
			COLMAP & 4762 & 169.9 & 173.33 & 190.09\\
			ORB-SLAM2 & \textbf{180} & \textbf{45.02} & \textbf{27.73} & \textbf{64.95}\\
			\bottomrule
	\end{tabular}}
	\caption{COLMAP vs. ORB-SLAM2 in accuracy and time.}
	\label{tab:colmap-orb}
\end{table}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/tables/gradEth.tex <==
\begin{table}[h]
	\begin{center}
		\footnotesize
		\begin{tabular}{lcccc}
			\toprule
			Model & $L_1^{Rel} \downarrow$ & $\delta_{1.25} \downarrow$ &  $\delta^2_{1.25} \downarrow$ & $\delta^3_{1.25} \downarrow$ \\
			\midrule
			MiDaS \cite{ranftl2019towards} &  0.2339 & 0.3254 & 0.1410 &  0.0779 \\
			CVDE \cite{CVDE} & 0.2171 & 0.2730 & 0.0960 & 0.0507 \\
			\midrule
			CVDE + $\mathcal{L}^\textit{MS}$ &  0.2165 & 0.2807 & \textbf{0.0921} & 0.0435 \\
			CVDE + $\mathcal{L}^\textit{C}$ &  \underline{\textbf{0.2143}} &  \underline{\textbf{0.2692}} &  \underline{0.0929} & \underline{0.0434}\\
			\bottomrule
		\end{tabular}
	\end{center}
	\caption{Quantitative evaluation of the proposed gradient-based losses on the ETH3D SLAM dataset. Our multi-scale gradient loss, $\mathcal{L}^\textit{MS}$, and the contrastive loss, $\mathcal{L}^\textit{C}$, outperform MiDaS and CVDE in $L_1^{Rel}$ and $\delta^2_{1.25}$ and in all metrics, respectively.}
	\label{tab:grad_eth}
\end{table}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/tables/stereoEval.tex <==
\begin{table}[h]
	\centering
	\footnotesize
	\begin{tabular}{lcc}
		\toprule
		Model & $L_1^{photo} \downarrow$ & $L_2^{photo} \downarrow$ \\
		\midrule
		LEAStereo \cite{cheng2020hierarchical} &  0.1989 & 0.0985  \\
		CVDE \cite{CVDE} & 0.1850  & 0.0954  \\
		\midrule
		Ours, $\mathcal{L}^\textit{LR}$ & 0.1721 & 0.0889 \\
		Ours, $\mathcal{L}^\textit{T}$  & 0.1350 & 0.0617 \\
		Ours, $\mathcal{L}^\textit{T}$, $\mathcal{L}^\textit{C}$ & 0.1214 & 0.0514 \\
		Ours, $\mathcal{L}^\textit{T}$, $\mathcal{L}^\textit{C}$, $\mathcal{L}^\textit{LR}$: \textbf{ECSV}  & \textbf{0.1010}  & \textbf{0.0440} \\
		\bottomrule
	\end{tabular}
	\caption{Quantitative evaluation on the KITTI odometry dataset. LEAStereo \cite{cheng2020hierarchical} is an image-based stereo model. CVDE \cite{CVDE} and our models are TTT approaches. Note that we use the losses to fine-tune the \emph{stereo} model \cite{cheng2020hierarchical}, LEAStereo. $L_1^{photo}$ and $L_2^{photo}$ are computed based on eq. \ref{eq:photometric}. Our comprehensive model (ECSV) outperforms CVDE by a large margin.}
	\label{tab:stereo_eval}
\end{table}


==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/tables/timeVcl.tex <==
\begin{table}[h]
	\footnotesize
	\centering
	\begin{tabular}{lc}
		\toprule
		Model & Time ($s$), on KITTI\\
		\midrule
		CVDE \cite{CVDE} &   6936 (\emph{mono})\\
		\midrule
		CVDE \cite{CVDE} + $\mathcal{L}^\textit{C}$ &  6949 (\emph{mono}) \\
		Ours, $\mathcal{L}^\textit{T}$ &   2850 (\emph{stereo}) \\
		Ours, $\mathcal{L}^\textit{LR}$ & \textbf{1200} (\emph{stereo})\\
		Ours, $\mathcal{L}^\textit{T}$, $\mathcal{L}^\textit{C}$, $\mathcal{L}^\textit{LR}$: \textbf{ECSV} & \underline{3180} (\emph{stereo}) \\
		\bottomrule
	\end{tabular}
	\caption{Timing comparison. \quotes{mono} and \quotes{stereo} denote fine-tuning the monocular (MiDaS) and stereo (LEAStereo) models in the TTT process, respectively. Compared to the mono-based TTT method, \ie CVDE, our stereo-based model, ECSV, requires less computation time. }
	\label{tab:time_vcl}
\end{table}

==> RAW_Final_Arxiv_Edge-aware Consistent Stereo Video Depth Estimation/tables/vclEval.tex <==
\begin{table}[h]
	\begin{center}
		\footnotesize
		\begin{tabular}{lcccc}
			\toprule
			Model & $L_1^{Rel} \downarrow$ & $\delta_{1.25} \downarrow$ &  $\delta^2_{1.25} \downarrow$ & $\delta^3_{1.25} \downarrow$\\
			\midrule
			MiDaS \cite{ranftl2019towards} &  0.2339 & 0.3254 & 0.1410 &  0.0779 \\
			Ours, $\mathcal{L}^\textit{LR}$ (\emph{mono})  & 0.2302 &  0.2956 & 0.1264 & 0.0634 \\
			\midrule
			CVDE \cite{CVDE} (\emph{mono}) & 0.2171 & 0.2730 & 0.0960 & 0.0507 \\
			Ours, $\mathcal{L}^\textit{LR}$, $\mathcal{L}^\textit{T}$ (\emph{mono}) & \textbf{0.2151} & \textbf{0.2520}  & \textbf{0.0920} & \textbf{0.0491} \\
			\bottomrule
		\end{tabular}
	\end{center}
	\caption{Quantitative evaluation of our proposed left-right consistency loss on the ETH3D dataset. Note that MiDaS and \quotes{Ours, $\mathcal{L}^\textit{LR}$} use per-frame estimation without applying geometric consistency across time. \quotes{mono} denote fine-tuning the monocular model, \ie MiDaS in the TTT process.}
	\label{tab:vcl_eval}
\end{table}
